The Uniqueness of LLaMA3-70B Series with Per-Channel Quantization

We have observed a distinctive quantization-related behavior in the LLaMA3/3.1-70B models that is absent in both the LLaMA2-70B and LLaMA3/3.1/3.2-1B/3B/8B/405B models. Quantization is a crucial technique for deploying large language models (LLMs) efficiently. The impact of W8A8 post-training quantization on model accuracy, especially on the recently released LLaMA3/3.1 model series, remains contentious. In this paper, we explore three key questions: What makes the LLaMA3-70B model series uniquely vulnerable to quantization? Why is this the case? And how can the issue be addressed? We empirically investigate multiple LLMs featured on an open LLM leaderboard, discovering that the LLaMA3-70B model series have a unique accuracy degradation behavior with W8A8 per-channel post-training quantization. In contrast, other model series such as LLaMA2, LLaMA3/3.1-8B, LLaMA3.2, Qwen, Mixtral, Mistral, Phi-3, and Falcon demonstrate robust performance with W8A8. Contrary to previous assertions attributing degradation to the large dynamic range of activations, our findings indicate that the weight distribution of the LLaMA3-70B is the primary factor behind the vulnerability. By meticulously analyzing the distinct characteristics of weight distributions across Transformer blocks, we propose two solutions that make different tradeoffs in hardware/software overhead. First, we propose a mixed strategy where less than 3\% of the layers employ finer per-group W8A8 quantization granularity. Second, we introduce a bi-smoothing strategy that balances quantization errors between weights and activations while maintaining per-channel quantization throughout. Experimental results demonstrate that both strategies effectively preserve the accuracy of the entire LLaMA3-70B model series under W8A8 quantization, achieving performance on par with their FP16 counterparts.

==> bibliography.tex <==
\begin{thebibliography}{44}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Vaswani et~al.(2023)Vaswani, Shazeer, Parmar, Uszkoreit, Jones, Gomez, Kaiser, and Polosukhin]{vaswani2023attentionneed}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones, Aidan~N. Gomez, Lukasz Kaiser, and Illia Polosukhin.
\newblock Attention is all you need, 2023.
\newblock URL \url{https://arxiv.org/abs/1706.03762}.

\bibitem[Brown et~al.(2020)Brown, Mann, Ryder, Subbiah, Kaplan, Dhariwal, Neelakantan, Shyam, Sastry, Askell, Agarwal, Herbert-Voss, Krueger, Henighan, Child, Ramesh, Ziegler, Wu, Winter, Hesse, Chen, Sigler, Litwin, Gray, Chess, Clark, Berner, McCandlish, Radford, Sutskever, and Amodei]{brown2020languagemodelsfewshotlearners}
Tom~B. Brown, Benjamin Mann, Nick Ryder, Melanie Subbiah, Jared Kaplan, Prafulla Dhariwal, Arvind Neelakantan, Pranav Shyam, Girish Sastry, Amanda Askell, Sandhini Agarwal, Ariel Herbert-Voss, Gretchen Krueger, Tom Henighan, Rewon Child, Aditya Ramesh, Daniel~M. Ziegler, Jeffrey Wu, Clemens Winter, Christopher Hesse, Mark Chen, Eric Sigler, Mateusz Litwin, Scott Gray, Benjamin Chess, Jack Clark, Christopher Berner, Sam McCandlish, Alec Radford, Ilya Sutskever, and Dario Amodei.
\newblock Language models are few-shot learners, 2020.
\newblock URL \url{https://arxiv.org/abs/2005.14165}.

\bibitem[Devlin et~al.(2019)Devlin, Chang, Lee, and Toutanova]{devlin2019bertpretrainingdeepbidirectional}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova.
\newblock Bert: Pre-training of deep bidirectional transformers for language understanding, 2019.
\newblock URL \url{https://arxiv.org/abs/1810.04805}.

\bibitem[Liu et~al.(2019)Liu, Ott, Goyal, Du, Joshi, Chen, Levy, Lewis, Zettlemoyer, and Stoyanov]{liu2019robertarobustlyoptimizedbert}
Yinhan Liu, Myle Ott, Naman Goyal, Jingfei Du, Mandar Joshi, Danqi Chen, Omer Levy, Mike Lewis, Luke Zettlemoyer, and Veselin Stoyanov.
\newblock Roberta: A robustly optimized bert pretraining approach, 2019.
\newblock URL \url{https://arxiv.org/abs/1907.11692}.

\bibitem[Touvron et~al.(2023)Touvron, Lavril, Izacard, Martinet, Lachaux, Lacroix, Rozière, Goyal, Hambro, Azhar, Rodriguez, Joulin, Grave, and Lample]{touvron2023llamaopenefficientfoundation}
Hugo Touvron, Thibaut Lavril, Gautier Izacard, Xavier Martinet, Marie-Anne Lachaux, Timothée Lacroix, Baptiste Rozière, Naman Goyal, Eric Hambro, Faisal Azhar, Aurelien Rodriguez, Armand Joulin, Edouard Grave, and Guillaume Lample.
\newblock Llama: Open and efficient foundation language models, 2023.
\newblock URL \url{https://arxiv.org/abs/2302.13971}.

\bibitem[Kaplan et~al.(2020)Kaplan, McCandlish, Henighan, Brown, Chess, Child, Gray, Radford, Wu, and Amodei]{kaplan2020scalinglawsneurallanguage}
Jared Kaplan, Sam McCandlish, Tom Henighan, Tom~B. Brown, Benjamin Chess, Rewon Child, Scott Gray, Alec Radford, Jeffrey Wu, and Dario Amodei.
\newblock Scaling laws for neural language models, 2020.
\newblock URL \url{https://arxiv.org/abs/2001.08361}.

\bibitem[Gholami et~al.(2021)Gholami, Kim, Dong, Yao, Mahoney, and Keutzer]{gholami2021surveyquantizationmethodsefficient}
Amir Gholami, Sehoon Kim, Zhen Dong, Zhewei Yao, Michael~W. Mahoney, and Kurt Keutzer.
\newblock A survey of quantization methods for efficient neural network inference, 2021.
\newblock URL \url{https://arxiv.org/abs/2103.13630}.

\bibitem[Zafrir et~al.(2019)Zafrir, Boudoukh, Izsak, and Wasserblat]{Zafrir_2019}
Ofir Zafrir, Guy Boudoukh, Peter Izsak, and Moshe Wasserblat.
\newblock Q8bert: Quantized 8bit bert.
\newblock In \emph{2019 Fifth Workshop on Energy Efficient Machine Learning and Cognitive Computing - NeurIPS Edition (EMC2-NIPS)}. IEEE, December 2019.
\newblock \doi{10.1109/emc2-nips53020.2019.00016}.
\newblock URL \url{http://dx.doi.org/10.1109/EMC2-NIPS53020.2019.00016}.

\bibitem[Wang et~al.(2023)Wang, Ma, Dong, Huang, Wang, Ma, Yang, Wang, Wu, and Wei]{wang2023bitnetscaling1bittransformers}
Hongyu Wang, Shuming Ma, Li~Dong, Shaohan Huang, Huaijie Wang, Lingxiao Ma, Fan Yang, Ruiping Wang, Yi~Wu, and Furu Wei.
\newblock Bitnet: Scaling 1-bit transformers for large language models, 2023.
\newblock URL \url{https://arxiv.org/abs/2310.11453}.

\bibitem[HuggingFace(2024)]{open-llm-leaderboard}
HuggingFace.
\newblock Open llm leaderboard.
\newblock \url{https://huggingface.co/spaces/open-llm-leaderboard/open_llm_leaderboard}, 2024.

\bibitem[Dubey et~al.(2024)Dubey, Jauhri, Pandey, Kadian, Al-Dahle, Letman, Mathur, Schelten, Yang, Fan, Goyal, Hartshorn, Yang, Mitra, Sravankumar, Korenev, Hinsvark, Rao, Zhang, Rodriguez, Gregerson, Spataru, Roziere, Biron, Tang, Chern, Caucheteux, Nayak, Bi, Marra, McConnell, Keller, Touret, Wu, Wong, Ferrer, Nikolaidis, Allonsius, Song, Pintz, Livshits, Esiobu, Choudhary, Mahajan, Garcia-Olano, Perino, Hupkes, Lakomkin, AlBadawy, Lobanova, Dinan, Smith, Radenovic, Zhang, Synnaeve, Lee, Anderson, Nail, Mialon, Pang, Cucurell, Nguyen, Korevaar, Xu, Touvron, Zarov, Ibarra, Kloumann, Misra, Evtimov, Copet, Lee, Geffert, Vranes, Park, Mahadeokar, Shah, van~der Linde, Billock, Hong, Lee, Fu, Chi, Huang, Liu, Wang, Yu, Bitton, Spisak, Park, Rocca, Johnstun, Saxe, Jia, Alwala, Upasani, Plawiak, Li, Heafield, Stone, El-Arini, Iyer, Malik, Chiu, Bhalla, Rantala-Yeary, van~der Maaten, Chen, Tan, Jenkins, Martin, Madaan, Malo, Blecher, Landzaat, de~Oliveira, Muzzi, Pasupuleti, Singh, Paluri, Kardas, Oldham, Rita,
  Pavlova, Kambadur, Lewis, Si, Singh, Hassan, Goyal, Torabi, Bashlykov, Bogoychev, Chatterji, Duchenne, Çelebi, Alrassy, Zhang, Li, Vasic, Weng, Bhargava, Dubal, Krishnan, Koura, Xu, He, Dong, Srinivasan, Ganapathy, Calderer, Cabral, Stojnic, Raileanu, Girdhar, Patel, Sauvestre, Polidoro, Sumbaly, Taylor, Silva, Hou, Wang, Hosseini, Chennabasappa, Singh, Bell, Kim, Edunov, Nie, Narang, Raparthy, Shen, Wan, Bhosale, Zhang, Vandenhende, Batra, Whitman, Sootla, Collot, Gururangan, Borodinsky, Herman, Fowler, Sheasha, Georgiou, Scialom, Speckbacher, Mihaylov, Xiao, Karn, Goswami, Gupta, Ramanathan, Kerkez, Gonguet, Do, Vogeti, Petrovic, Chu, Xiong, Fu, Meers, Martinet, Wang, Tan, Xie, Jia, Wang, Goldschlag, Gaur, Babaei, Wen, Song, Zhang, Li, Mao, Coudert, Yan, Chen, Papakipos, Singh, Grattafiori, Jain, Kelsey, Shajnfeld, Gangidi, Victoria, Goldstand, Menon, Sharma, Boesenberg, Vaughan, Baevski, Feinstein, Kallet, Sangani, Yunus, Lupu, Alvarado, Caples, Gu, Ho, Poulton, Ryan, Ramchandani, Franco, Saraf,
  Chowdhury, Gabriel, Bharambe, Eisenman, Yazdan, James, Maurer, Leonhardi, Huang, Loyd, Paola, Paranjape, Liu, Wu, Ni, Hancock, Wasti, Spence, Stojkovic, Gamido, Montalvo, Parker, Burton, Mejia, Wang, Kim, Zhou, Hu, Chu, Cai, Tindal, Feichtenhofer, Civin, Beaty, Kreymer, Li, Wyatt, Adkins, Xu, Testuggine, David, Parikh, Liskovich, Foss, Wang, Le, Holland, Dowling, Jamil, Montgomery, Presani, Hahn, Wood, Brinkman, Arcaute, Dunbar, Smothers, Sun, Kreuk, Tian, Ozgenel, Caggioni, Guzmán, Kanayet, Seide, Florez, Schwarz, Badeer, Swee, Halpern, Thattai, Herman, Sizov, Guangyi, Zhang, Lakshminarayanan, Shojanazeri, Zou, Wang, Zha, Habeeb, Rudolph, Suk, Aspegren, Goldman, Molybog, Tufanov, Veliche, Gat, Weissman, Geboski, Kohli, Asher, Gaya, Marcus, Tang, Chan, Zhen, Reizenstein, Teboul, Zhong, Jin, Yang, Cummings, Carvill, Shepard, McPhie, Torres, Ginsburg, Wang, Wu, U, Saxena, Prasad, Khandelwal, Zand, Matosich, Veeraraghavan, Michelena, Li, Huang, Chawla, Lakhotia, Huang, Chen, Garg, A, Silva, Bell, Zhang, Guo,
  Yu, Moshkovich, Wehrstedt, Khabsa, Avalani, Bhatt, Tsimpoukelli, Mankus, Hasson, Lennie, Reso, Groshev, Naumov, Lathi, Keneally, Seltzer, Valko, Restrepo, Patel, Vyatskov, Samvelyan, Clark, Macey, Wang, Hermoso, Metanat, Rastegari, Bansal, Santhanam, Parks, White, Bawa, Singhal, Egebo, Usunier, Laptev, Dong, Zhang, Cheng, Chernoguz, Hart, Salpekar, Kalinli, Kent, Parekh, Saab, Balaji, Rittner, Bontrager, Roux, Dollar, Zvyagina, Ratanchandani, Yuvraj, Liang, Alao, Rodriguez, Ayub, Murthy, Nayani, Mitra, Li, Hogan, Battey, Wang, Maheswari, Howes, Rinott, Bondu, Datta, Chugh, Hunt, Dhillon, Sidorov, Pan, Verma, Yamamoto, Ramaswamy, Lindsay, Lindsay, Feng, Lin, Zha, Shankar, Zhang, Zhang, Wang, Agarwal, Sajuyigbe, Chintala, Max, Chen, Kehoe, Satterfield, Govindaprasad, Gupta, Cho, Virk, Subramanian, Choudhury, Goldman, Remez, Glaser, Best, Kohler, Robinson, Li, Zhang, Matthews, Chou, Shaked, Vontimitta, Ajayi, Montanez, Mohan, Kumar, Mangla, Ionescu, Poenaru, Mihailescu, Ivanov, Li, Wang, Jiang, Bouaziz,
  Constable, Tang, Wang, Wu, Wang, Xia, Wu, Gao, Chen, Hu, Jia, Qi, Li, Zhang, Zhang, Adi, Nam, Yu, Wang, Hao, Qian, He, Rait, DeVito, Rosnbrick, Wen, Yang, and Zhao]{dubey2024llama3herdmodels}
Abhimanyu Dubey, Abhinav Jauhri, Abhinav Pandey, Abhishek Kadian, Ahmad Al-Dahle, Aiesha Letman, Akhil Mathur, Alan Schelten, Amy Yang, Angela Fan, Anirudh Goyal, Anthony Hartshorn, Aobo Yang, Archi Mitra, Archie Sravankumar, Artem Korenev, Arthur Hinsvark, Arun Rao, Aston Zhang, Aurelien Rodriguez, Austen Gregerson, Ava Spataru, Baptiste Roziere, Bethany Biron, Binh Tang, Bobbie Chern, Charlotte Caucheteux, Chaya Nayak, Chloe Bi, Chris Marra, Chris McConnell, Christian Keller, Christophe Touret, Chunyang Wu, Corinne Wong, Cristian~Canton Ferrer, Cyrus Nikolaidis, Damien Allonsius, Daniel Song, Danielle Pintz, Danny Livshits, David Esiobu, Dhruv Choudhary, Dhruv Mahajan, Diego Garcia-Olano, Diego Perino, Dieuwke Hupkes, Egor Lakomkin, Ehab AlBadawy, Elina Lobanova, Emily Dinan, Eric~Michael Smith, Filip Radenovic, Frank Zhang, Gabriel Synnaeve, Gabrielle Lee, Georgia~Lewis Anderson, Graeme Nail, Gregoire Mialon, Guan Pang, Guillem Cucurell, Hailey Nguyen, Hannah Korevaar, Hu~Xu, Hugo Touvron, Iliyan Zarov,
  Imanol~Arrieta Ibarra, Isabel Kloumann, Ishan Misra, Ivan Evtimov, Jade Copet, Jaewon Lee, Jan Geffert, Jana Vranes, Jason Park, Jay Mahadeokar, Jeet Shah, Jelmer van~der Linde, Jennifer Billock, Jenny Hong, Jenya Lee, Jeremy Fu, Jianfeng Chi, Jianyu Huang, Jiawen Liu, Jie Wang, Jiecao Yu, Joanna Bitton, Joe Spisak, Jongsoo Park, Joseph Rocca, Joshua Johnstun, Joshua Saxe, Junteng Jia, Kalyan~Vasuden Alwala, Kartikeya Upasani, Kate Plawiak, Ke~Li, Kenneth Heafield, Kevin Stone, Khalid El-Arini, Krithika Iyer, Kshitiz Malik, Kuenley Chiu, Kunal Bhalla, Lauren Rantala-Yeary, Laurens van~der Maaten, Lawrence Chen, Liang Tan, Liz Jenkins, Louis Martin, Lovish Madaan, Lubo Malo, Lukas Blecher, Lukas Landzaat, Luke de~Oliveira, Madeline Muzzi, Mahesh Pasupuleti, Mannat Singh, Manohar Paluri, Marcin Kardas, Mathew Oldham, Mathieu Rita, Maya Pavlova, Melanie Kambadur, Mike Lewis, Min Si, Mitesh~Kumar Singh, Mona Hassan, Naman Goyal, Narjes Torabi, Nikolay Bashlykov, Nikolay Bogoychev, Niladri Chatterji, Olivier
  Duchenne, Onur Çelebi, Patrick Alrassy, Pengchuan Zhang, Pengwei Li, Petar Vasic, Peter Weng, Prajjwal Bhargava, Pratik Dubal, Praveen Krishnan, Punit~Singh Koura, Puxin Xu, Qing He, Qingxiao Dong, Ragavan Srinivasan, Raj Ganapathy, Ramon Calderer, Ricardo~Silveira Cabral, Robert Stojnic, Roberta Raileanu, Rohit Girdhar, Rohit Patel, Romain Sauvestre, Ronnie Polidoro, Roshan Sumbaly, Ross Taylor, Ruan Silva, Rui Hou, Rui Wang, Saghar Hosseini, Sahana Chennabasappa, Sanjay Singh, Sean Bell, Seohyun~Sonia Kim, Sergey Edunov, Shaoliang Nie, Sharan Narang, Sharath Raparthy, Sheng Shen, Shengye Wan, Shruti Bhosale, Shun Zhang, Simon Vandenhende, Soumya Batra, Spencer Whitman, Sten Sootla, Stephane Collot, Suchin Gururangan, Sydney Borodinsky, Tamar Herman, Tara Fowler, Tarek Sheasha, Thomas Georgiou, Thomas Scialom, Tobias Speckbacher, Todor Mihaylov, Tong Xiao, Ujjwal Karn, Vedanuj Goswami, Vibhor Gupta, Vignesh Ramanathan, Viktor Kerkez, Vincent Gonguet, Virginie Do, Vish Vogeti, Vladan Petrovic, Weiwei Chu,
  Wenhan Xiong, Wenyin Fu, Whitney Meers, Xavier Martinet, Xiaodong Wang, Xiaoqing~Ellen Tan, Xinfeng Xie, Xuchao Jia, Xuewei Wang, Yaelle Goldschlag, Yashesh Gaur, Yasmine Babaei, Yi~Wen, Yiwen Song, Yuchen Zhang, Yue Li, Yuning Mao, Zacharie~Delpierre Coudert, Zheng Yan, Zhengxing Chen, Zoe Papakipos, Aaditya Singh, Aaron Grattafiori, Abha Jain, Adam Kelsey, Adam Shajnfeld, Adithya Gangidi, Adolfo Victoria, Ahuva Goldstand, Ajay Menon, Ajay Sharma, Alex Boesenberg, Alex Vaughan, Alexei Baevski, Allie Feinstein, Amanda Kallet, Amit Sangani, Anam Yunus, Andrei Lupu, Andres Alvarado, Andrew Caples, Andrew Gu, Andrew Ho, Andrew Poulton, Andrew Ryan, Ankit Ramchandani, Annie Franco, Aparajita Saraf, Arkabandhu Chowdhury, Ashley Gabriel, Ashwin Bharambe, Assaf Eisenman, Azadeh Yazdan, Beau James, Ben Maurer, Benjamin Leonhardi, Bernie Huang, Beth Loyd, Beto~De Paola, Bhargavi Paranjape, Bing Liu, Bo~Wu, Boyu Ni, Braden Hancock, Bram Wasti, Brandon Spence, Brani Stojkovic, Brian Gamido, Britt Montalvo, Carl
  Parker, Carly Burton, Catalina Mejia, Changhan Wang, Changkyu Kim, Chao Zhou, Chester Hu, Ching-Hsiang Chu, Chris Cai, Chris Tindal, Christoph Feichtenhofer, Damon Civin, Dana Beaty, Daniel Kreymer, Daniel Li, Danny Wyatt, David Adkins, David Xu, Davide Testuggine, Delia David, Devi Parikh, Diana Liskovich, Didem Foss, Dingkang Wang, Duc Le, Dustin Holland, Edward Dowling, Eissa Jamil, Elaine Montgomery, Eleonora Presani, Emily Hahn, Emily Wood, Erik Brinkman, Esteban Arcaute, Evan Dunbar, Evan Smothers, Fei Sun, Felix Kreuk, Feng Tian, Firat Ozgenel, Francesco Caggioni, Francisco Guzmán, Frank Kanayet, Frank Seide, Gabriela~Medina Florez, Gabriella Schwarz, Gada Badeer, Georgia Swee, Gil Halpern, Govind Thattai, Grant Herman, Grigory Sizov, Guangyi, Zhang, Guna Lakshminarayanan, Hamid Shojanazeri, Han Zou, Hannah Wang, Hanwen Zha, Haroun Habeeb, Harrison Rudolph, Helen Suk, Henry Aspegren, Hunter Goldman, Igor Molybog, Igor Tufanov, Irina-Elena Veliche, Itai Gat, Jake Weissman, James Geboski, James Kohli,
  Japhet Asher, Jean-Baptiste Gaya, Jeff Marcus, Jeff Tang, Jennifer Chan, Jenny Zhen, Jeremy Reizenstein, Jeremy Teboul, Jessica Zhong, Jian Jin, Jingyi Yang, Joe Cummings, Jon Carvill, Jon Shepard, Jonathan McPhie, Jonathan Torres, Josh Ginsburg, Junjie Wang, Kai Wu, Kam~Hou U, Karan Saxena, Karthik Prasad, Kartikay Khandelwal, Katayoun Zand, Kathy Matosich, Kaushik Veeraraghavan, Kelly Michelena, Keqian Li, Kun Huang, Kunal Chawla, Kushal Lakhotia, Kyle Huang, Lailin Chen, Lakshya Garg, Lavender A, Leandro Silva, Lee Bell, Lei Zhang, Liangpeng Guo, Licheng Yu, Liron Moshkovich, Luca Wehrstedt, Madian Khabsa, Manav Avalani, Manish Bhatt, Maria Tsimpoukelli, Martynas Mankus, Matan Hasson, Matthew Lennie, Matthias Reso, Maxim Groshev, Maxim Naumov, Maya Lathi, Meghan Keneally, Michael~L. Seltzer, Michal Valko, Michelle Restrepo, Mihir Patel, Mik Vyatskov, Mikayel Samvelyan, Mike Clark, Mike Macey, Mike Wang, Miquel~Jubert Hermoso, Mo~Metanat, Mohammad Rastegari, Munish Bansal, Nandhini Santhanam, Natascha
  Parks, Natasha White, Navyata Bawa, Nayan Singhal, Nick Egebo, Nicolas Usunier, Nikolay~Pavlovich Laptev, Ning Dong, Ning Zhang, Norman Cheng, Oleg Chernoguz, Olivia Hart, Omkar Salpekar, Ozlem Kalinli, Parkin Kent, Parth Parekh, Paul Saab, Pavan Balaji, Pedro Rittner, Philip Bontrager, Pierre Roux, Piotr Dollar, Polina Zvyagina, Prashant Ratanchandani, Pritish Yuvraj, Qian Liang, Rachad Alao, Rachel Rodriguez, Rafi Ayub, Raghotham Murthy, Raghu Nayani, Rahul Mitra, Raymond Li, Rebekkah Hogan, Robin Battey, Rocky Wang, Rohan Maheswari, Russ Howes, Ruty Rinott, Sai~Jayesh Bondu, Samyak Datta, Sara Chugh, Sara Hunt, Sargun Dhillon, Sasha Sidorov, Satadru Pan, Saurabh Verma, Seiji Yamamoto, Sharadh Ramaswamy, Shaun Lindsay, Shaun Lindsay, Sheng Feng, Shenghao Lin, Shengxin~Cindy Zha, Shiva Shankar, Shuqiang Zhang, Shuqiang Zhang, Sinong Wang, Sneha Agarwal, Soji Sajuyigbe, Soumith Chintala, Stephanie Max, Stephen Chen, Steve Kehoe, Steve Satterfield, Sudarshan Govindaprasad, Sumit Gupta, Sungmin Cho, Sunny
  Virk, Suraj Subramanian, Sy~Choudhury, Sydney Goldman, Tal Remez, Tamar Glaser, Tamara Best, Thilo Kohler, Thomas Robinson, Tianhe Li, Tianjun Zhang, Tim Matthews, Timothy Chou, Tzook Shaked, Varun Vontimitta, Victoria Ajayi, Victoria Montanez, Vijai Mohan, Vinay~Satish Kumar, Vishal Mangla, Vlad Ionescu, Vlad Poenaru, Vlad~Tiberiu Mihailescu, Vladimir Ivanov, Wei Li, Wenchen Wang, Wenwen Jiang, Wes Bouaziz, Will Constable, Xiaocheng Tang, Xiaofang Wang, Xiaojian Wu, Xiaolan Wang, Xide Xia, Xilun Wu, Xinbo Gao, Yanjun Chen, Ye~Hu, Ye~Jia, Ye~Qi, Yenda Li, Yilin Zhang, Ying Zhang, Yossi Adi, Youngjin Nam, Yu, Wang, Yuchen Hao, Yundi Qian, Yuzi He, Zach Rait, Zachary DeVito, Zef Rosnbrick, Zhaoduo Wen, Zhenyu Yang, and Zhiwei Zhao.
\newblock The llama 3 herd of models, 2024.
\newblock URL \url{https://arxiv.org/abs/2407.21783}.

\bibitem[Jiang et~al.(2023)Jiang, Sablayrolles, Mensch, Bamford, Chaplot, de~las Casas, Bressand, Lengyel, Lample, Saulnier, Lavaud, Lachaux, Stock, Scao, Lavril, Wang, Lacroix, and Sayed]{jiang2023mistral7b}
Albert~Q. Jiang, Alexandre Sablayrolles, Arthur Mensch, Chris Bamford, Devendra~Singh Chaplot, Diego de~las Casas, Florian Bressand, Gianna Lengyel, Guillaume Lample, Lucile Saulnier, Lélio~Renard Lavaud, Marie-Anne Lachaux, Pierre Stock, Teven~Le Scao, Thibaut Lavril, Thomas Wang, Timothée Lacroix, and William~El Sayed.
\newblock Mistral 7b, 2023.
\newblock URL \url{https://arxiv.org/abs/2310.06825}.

\bibitem[Jiang et~al.(2024)Jiang, Sablayrolles, Roux, Mensch, Savary, Bamford, Chaplot, de~las Casas, Hanna, Bressand, Lengyel, Bour, Lample, Lavaud, Saulnier, Lachaux, Stock, Subramanian, Yang, Antoniak, Scao, Gervet, Lavril, Wang, Lacroix, and Sayed]{jiang2024mixtralexperts}
Albert~Q. Jiang, Alexandre Sablayrolles, Antoine Roux, Arthur Mensch, Blanche Savary, Chris Bamford, Devendra~Singh Chaplot, Diego de~las Casas, Emma~Bou Hanna, Florian Bressand, Gianna Lengyel, Guillaume Bour, Guillaume Lample, Lélio~Renard Lavaud, Lucile Saulnier, Marie-Anne Lachaux, Pierre Stock, Sandeep Subramanian, Sophia Yang, Szymon Antoniak, Teven~Le Scao, Théophile Gervet, Thibaut Lavril, Thomas Wang, Timothée Lacroix, and William~El Sayed.
\newblock Mixtral of experts, 2024.
\newblock URL \url{https://arxiv.org/abs/2401.04088}.

\bibitem[Yang et~al.(2024)Yang, Yang, Hui, Zheng, Yu, Zhou, Li, Li, Liu, Huang, Dong, Wei, Lin, Tang, Wang, Yang, Tu, Zhang, Ma, Yang, Xu, Zhou, Bai, He, Lin, Dang, Lu, Chen, Yang, Li, Xue, Ni, Zhang, Wang, Peng, Men, Gao, Lin, Wang, Bai, Tan, Zhu, Li, Liu, Ge, Deng, Zhou, Ren, Zhang, Wei, Ren, Liu, Fan, Yao, Zhang, Wan, Chu, Liu, Cui, Zhang, Guo, and Fan]{yang2024qwen2technicalreport}
An~Yang, Baosong Yang, Binyuan Hui, Bo~Zheng, Bowen Yu, Chang Zhou, Chengpeng Li, Chengyuan Li, Dayiheng Liu, Fei Huang, Guanting Dong, Haoran Wei, Huan Lin, Jialong Tang, Jialin Wang, Jian Yang, Jianhong Tu, Jianwei Zhang, Jianxin Ma, Jianxin Yang, Jin Xu, Jingren Zhou, Jinze Bai, Jinzheng He, Junyang Lin, Kai Dang, Keming Lu, Keqin Chen, Kexin Yang, Mei Li, Mingfeng Xue, Na~Ni, Pei Zhang, Peng Wang, Ru~Peng, Rui Men, Ruize Gao, Runji Lin, Shijie Wang, Shuai Bai, Sinan Tan, Tianhang Zhu, Tianhao Li, Tianyu Liu, Wenbin Ge, Xiaodong Deng, Xiaohuan Zhou, Xingzhang Ren, Xinyu Zhang, Xipin Wei, Xuancheng Ren, Xuejing Liu, Yang Fan, Yang Yao, Yichang Zhang, Yu~Wan, Yunfei Chu, Yuqiong Liu, Zeyu Cui, Zhenru Zhang, Zhifang Guo, and Zhihao Fan.
\newblock Qwen2 technical report, 2024.
\newblock URL \url{https://arxiv.org/abs/2407.10671}.

\bibitem[Abdin et~al.(2024)Abdin, Jacobs, Awan, Aneja, Awadallah, Awadalla, Bach, Bahree, Bakhtiari, Bao, Behl, Benhaim, Bilenko, Bjorck, Bubeck, Cai, Cai, Mendes, Chen, Chaudhary, Chen, Chen, Chen, Chen, Chopra, Dai, Giorno, de~Rosa, Dixon, Eldan, Fragoso, Iter, Gao, Gao, Gao, Garg, Goswami, Gunasekar, Haider, Hao, Hewett, Huynh, Javaheripi, Jin, Kauffmann, Karampatziakis, Kim, Khademi, Kurilenko, Lee, Lee, Li, Li, Liang, Liden, Liu, Liu, Liu, Lin, Lin, Luo, Madan, Mazzola, Mitra, Modi, Nguyen, Norick, Patra, Perez-Becker, Portet, Pryzant, Qin, Radmilac, Rosset, Roy, Ruwase, Saarikivi, Saied, Salim, Santacroce, Shah, Shang, Sharma, Shukla, Song, Tanaka, Tupini, Wang, Wang, Wang, Wang, Ward, Wang, Witte, Wu, Wyatt, Xiao, Xu, Xu, Xu, Yadav, Yang, Yang, Yang, Yang, Yu, Yuan, Zhang, Zhang, Zhang, Zhang, Zhang, Zhang, Zhang, and Zhou]{abdin2024phi3technicalreporthighly}
Marah Abdin, Sam~Ade Jacobs, Ammar~Ahmad Awan, Jyoti Aneja, Ahmed Awadallah, Hany Awadalla, Nguyen Bach, Amit Bahree, Arash Bakhtiari, Jianmin Bao, Harkirat Behl, Alon Benhaim, Misha Bilenko, Johan Bjorck, Sébastien Bubeck, Qin Cai, Martin Cai, Caio César~Teodoro Mendes, Weizhu Chen, Vishrav Chaudhary, Dong Chen, Dongdong Chen, Yen-Chun Chen, Yi-Ling Chen, Parul Chopra, Xiyang Dai, Allie~Del Giorno, Gustavo de~Rosa, Matthew Dixon, Ronen Eldan, Victor Fragoso, Dan Iter, Mei Gao, Min Gao, Jianfeng Gao, Amit Garg, Abhishek Goswami, Suriya Gunasekar, Emman Haider, Junheng Hao, Russell~J. Hewett, Jamie Huynh, Mojan Javaheripi, Xin Jin, Piero Kauffmann, Nikos Karampatziakis, Dongwoo Kim, Mahoud Khademi, Lev Kurilenko, James~R. Lee, Yin~Tat Lee, Yuanzhi Li, Yunsheng Li, Chen Liang, Lars Liden, Ce~Liu, Mengchen Liu, Weishung Liu, Eric Lin, Zeqi Lin, Chong Luo, Piyush Madan, Matt Mazzola, Arindam Mitra, Hardik Modi, Anh Nguyen, Brandon Norick, Barun Patra, Daniel Perez-Becker, Thomas Portet, Reid Pryzant, Heyang
  Qin, Marko Radmilac, Corby Rosset, Sambudha Roy, Olatunji Ruwase, Olli Saarikivi, Amin Saied, Adil Salim, Michael Santacroce, Shital Shah, Ning Shang, Hiteshi Sharma, Swadheen Shukla, Xia Song, Masahiro Tanaka, Andrea Tupini, Xin Wang, Lijuan Wang, Chunyu Wang, Yu~Wang, Rachel Ward, Guanhua Wang, Philipp Witte, Haiping Wu, Michael Wyatt, Bin Xiao, Can Xu, Jiahang Xu, Weijian Xu, Sonali Yadav, Fan Yang, Jianwei Yang, Ziyi Yang, Yifan Yang, Donghan Yu, Lu~Yuan, Chengruidong Zhang, Cyril Zhang, Jianwen Zhang, Li~Lyna Zhang, Yi~Zhang, Yue Zhang, Yunan Zhang, and Xiren Zhou.
\newblock Phi-3 technical report: A highly capable language model locally on your phone, 2024.
\newblock URL \url{https://arxiv.org/abs/2404.14219}.

\bibitem[Almazrouei et~al.(2023)Almazrouei, Alobeidli, Alshamsi, Cappelli, Cojocaru, Debbah, Étienne Goffinet, Hesslow, Launay, Malartic, Mazzotta, Noune, Pannier, and Penedo]{almazrouei2023falconseriesopenlanguage}
Ebtesam Almazrouei, Hamza Alobeidli, Abdulaziz Alshamsi, Alessandro Cappelli, Ruxandra Cojocaru, Mérouane Debbah, Étienne Goffinet, Daniel Hesslow, Julien Launay, Quentin Malartic, Daniele Mazzotta, Badreddine Noune, Baptiste Pannier, and Guilherme Penedo.
\newblock The falcon series of open language models, 2023.
\newblock URL \url{https://arxiv.org/abs/2311.16867}.

\bibitem[Zellers et~al.(2019)Zellers, Holtzman, Bisk, Farhadi, and Choi]{zellers2019hellaswagmachinereallyfinish}
Rowan Zellers, Ari Holtzman, Yonatan Bisk, Ali Farhadi, and Yejin Choi.
\newblock Hellaswag: Can a machine really finish your sentence?, 2019.
\newblock URL \url{https://arxiv.org/abs/1905.07830}.

\bibitem[Bisk et~al.(2019)Bisk, Zellers, Bras, Gao, and Choi]{bisk2019piqareasoningphysicalcommonsense}
Yonatan Bisk, Rowan Zellers, Ronan~Le Bras, Jianfeng Gao, and Yejin Choi.
\newblock Piqa: Reasoning about physical commonsense in natural language, 2019.
\newblock URL \url{https://arxiv.org/abs/1911.11641}.

\bibitem[Mihaylov et~al.(2018)Mihaylov, Clark, Khot, and Sabharwal]{OpenBookQA2018}
Todor Mihaylov, Peter Clark, Tushar Khot, and Ashish Sabharwal.
\newblock Can a suit of armor conduct electricity? a new dataset for open book question answering.
\newblock In \emph{EMNLP}, 2018.

\bibitem[Clark et~al.(2018)Clark, Cowhey, Etzioni, Khot, Sabharwal, Schoenick, and Tafjord]{allenai:arc}
Peter Clark, Isaac Cowhey, Oren Etzioni, Tushar Khot, Ashish Sabharwal, Carissa Schoenick, and Oyvind Tafjord.
\newblock Think you have solved question answering? try arc, the ai2 reasoning challenge.
\newblock \emph{arXiv:1803.05457v1}, 2018.

\bibitem[Sakaguchi et~al.(2019)Sakaguchi, Bras, Bhagavatula, and Choi]{sakaguchi2019winograndeadversarialwinogradschema}
Keisuke Sakaguchi, Ronan~Le Bras, Chandra Bhagavatula, and Yejin Choi.
\newblock Winogrande: An adversarial winograd schema challenge at scale, 2019.
\newblock URL \url{https://arxiv.org/abs/1907.10641}.

\bibitem[Clark et~al.(2019)Clark, Lee, Chang, Kwiatkowski, Collins, and Toutanova]{clark2019boolqexploringsurprisingdifficulty}
Christopher Clark, Kenton Lee, Ming-Wei Chang, Tom Kwiatkowski, Michael Collins, and Kristina Toutanova.
\newblock Boolq: Exploring the surprising difficulty of natural yes/no questions, 2019.
\newblock URL \url{https://arxiv.org/abs/1905.10044}.

\bibitem[Hendrycks et~al.(2021{\natexlab{a}})Hendrycks, Burns, Basart, Zou, Mazeika, Song, and Steinhardt]{hendryckstest2021}
Dan Hendrycks, Collin Burns, Steven Basart, Andy Zou, Mantas Mazeika, Dawn Song, and Jacob Steinhardt.
\newblock Measuring massive multitask language understanding.
\newblock \emph{Proceedings of the International Conference on Learning Representations (ICLR)}, 2021{\natexlab{a}}.

\bibitem[Hendrycks et~al.(2021{\natexlab{b}})Hendrycks, Burns, Basart, Critch, Li, Song, and Steinhardt]{hendrycks2021ethics}
Dan Hendrycks, Collin Burns, Steven Basart, Andrew Critch, Jerry Li, Dawn Song, and Jacob Steinhardt.
\newblock Aligning ai with shared human values.
\newblock \emph{Proceedings of the International Conference on Learning Representations (ICLR)}, 2021{\natexlab{b}}.

\bibitem[Gao et~al.(2023)Gao, Tow, Abbasi, Biderman, Black, DiPofi, Foster, Golding, Hsu, Le~Noac'h, Li, McDonell, Muennighoff, Ociepa, Phang, Reynolds, Schoelkopf, Skowron, Sutawika, Tang, Thite, Wang, Wang, and Zou]{eval-harness}
Leo Gao, Jonathan Tow, Baber Abbasi, Stella Biderman, Sid Black, Anthony DiPofi, Charles Foster, Laurence Golding, Jeffrey Hsu, Alain Le~Noac'h, Haonan Li, Kyle McDonell, Niklas Muennighoff, Chris Ociepa, Jason Phang, Laria Reynolds, Hailey Schoelkopf, Aviya Skowron, Lintang Sutawika, Eric Tang, Anish Thite, Ben Wang, Kevin Wang, and Andy Zou.
\newblock A framework for few-shot language model evaluation, 12 2023.
\newblock URL \url{https://zenodo.org/records/10256836}.

\bibitem[Han et~al.(2016)Han, Mao, and Dally]{han2016deepcompressioncompressingdeep}
Song Han, Huizi Mao, and William~J. Dally.
\newblock Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding, 2016.
\newblock URL \url{https://arxiv.org/abs/1510.00149}.

\bibitem[Jacob et~al.(2017)Jacob, Kligys, Chen, Zhu, Tang, Howard, Adam, and Kalenichenko]{jacob2017quantizationtrainingneuralnetworks}
Benoit Jacob, Skirmantas Kligys, Bo~Chen, Menglong Zhu, Matthew Tang, Andrew Howard, Hartwig Adam, and Dmitry Kalenichenko.
\newblock Quantization and training of neural networks for efficient integer-arithmetic-only inference, 2017.
\newblock URL \url{https://arxiv.org/abs/1712.05877}.

\bibitem[Nagel et~al.(2019)Nagel, van Baalen, Blankevoort, and Welling]{nagel2019datafreequantizationweightequalization}
Markus Nagel, Mart van Baalen, Tijmen Blankevoort, and Max Welling.
\newblock Data-free quantization through weight equalization and bias correction, 2019.
\newblock URL \url{https://arxiv.org/abs/1906.04721}.

\bibitem[Bondarenko et~al.(2021)Bondarenko, Nagel, and Blankevoort]{bondarenko2021understandingovercomingchallengesefficient}
Yelysei Bondarenko, Markus Nagel, and Tijmen Blankevoort.
\newblock Understanding and overcoming the challenges of efficient transformer quantization, 2021.
\newblock URL \url{https://arxiv.org/abs/2109.12948}.

\bibitem[Wang et~al.(2019)Wang, Liu, Lin, Lin, and Han]{wang2019haqhardwareawareautomatedquantization}
Kuan Wang, Zhijian Liu, Yujun Lin, Ji~Lin, and Song Han.
\newblock Haq: Hardware-aware automated quantization with mixed precision, 2019.
\newblock URL \url{https://arxiv.org/abs/1811.08886}.

\bibitem[Bengio et~al.(2013)Bengio, Léonard, and Courville]{bengio2013estimatingpropagatinggradientsstochastic}
Yoshua Bengio, Nicholas Léonard, and Aaron Courville.
\newblock Estimating or propagating gradients through stochastic neurons for conditional computation, 2013.
\newblock URL \url{https://arxiv.org/abs/1308.3432}.

\bibitem[Dettmers et~al.(2022{\natexlab{a}})Dettmers, Lewis, Belkada, and Zettlemoyer]{dettmers2022llmint8}
Tim Dettmers, Mike Lewis, Younes Belkada, and Luke Zettlemoyer.
\newblock Llm.int8(): 8-bit matrix multiplication for transformers at scale, 2022{\natexlab{a}}.
\newblock URL \url{https://arxiv.org/abs/2208.07339}.

\bibitem[Frantar et~al.(2023)Frantar, Ashkboos, Hoefler, and Alistarh]{frantar2023gptq}
Elias Frantar, Saleh Ashkboos, Torsten Hoefler, and Dan Alistarh.
\newblock Gptq: Accurate post-training quantization for generative pre-trained transformers, 2023.
\newblock URL \url{https://arxiv.org/abs/2210.17323}.

\bibitem[Lin et~al.(2024{\natexlab{a}})Lin, Tang, Tang, Yang, Chen, Wang, Xiao, Dang, Gan, and Han]{lin2023awq}
Ji~Lin, Jiaming Tang, Haotian Tang, Shang Yang, Wei-Ming Chen, Wei-Chen Wang, Guangxuan Xiao, Xingyu Dang, Chuang Gan, and Song Han.
\newblock Awq: Activation-aware weight quantization for llm compression and acceleration.
\newblock In \emph{MLSys}, 2024{\natexlab{a}}.

\bibitem[Kim et~al.(2024)Kim, Hooper, Gholami, Dong, Li, Shen, Mahoney, and Keutzer]{kim2024squeezellmdenseandsparsequantization}
Sehoon Kim, Coleman Hooper, Amir Gholami, Zhen Dong, Xiuyu Li, Sheng Shen, Michael~W. Mahoney, and Kurt Keutzer.
\newblock Squeezellm: Dense-and-sparse quantization, 2024.
\newblock URL \url{https://arxiv.org/abs/2306.07629}.

\bibitem[Dettmers et~al.(2022{\natexlab{b}})Dettmers, Lewis, Belkada, and Zettlemoyer]{dettmers2022gptint}
Tim Dettmers, Mike Lewis, Younes Belkada, and Luke Zettlemoyer.
\newblock {GPT}3.int8(): 8-bit matrix multiplication for transformers at scale.
\newblock In Alice~H. Oh, Alekh Agarwal, Danielle Belgrave, and Kyunghyun Cho, editors, \emph{Advances in Neural Information Processing Systems}, 2022{\natexlab{b}}.
\newblock URL \url{https://openreview.net/forum?id=dXiGWqBoxaD}.

\bibitem[Wei et~al.(2023)Wei, Zhang, Zhang, Gong, Zhang, Zhang, Yu, and Liu]{wei2023outliersuppressionpushinglimit}
Xiuying Wei, Yunchen Zhang, Xiangguo Zhang, Ruihao Gong, Shanghang Zhang, Qi~Zhang, Fengwei Yu, and Xianglong Liu.
\newblock Outlier suppression: Pushing the limit of low-bit transformer language models, 2023.
\newblock URL \url{https://arxiv.org/abs/2209.13325}.

\bibitem[Xiao et~al.(2024)Xiao, Lin, Seznec, Wu, Demouth, and Han]{xiao2024smoothquantaccurateefficientposttraining}
Guangxuan Xiao, Ji~Lin, Mickael Seznec, Hao Wu, Julien Demouth, and Song Han.
\newblock Smoothquant: Accurate and efficient post-training quantization for large language models, 2024.
\newblock URL \url{https://arxiv.org/abs/2211.10438}.

\bibitem[Lin et~al.(2024{\natexlab{b}})Lin, Tang, Yang, Zhang, Xiao, Gan, and Han]{lin2024qservew4a8kv4quantizationcodesign}
Yujun Lin, Haotian Tang, Shang Yang, Zhekai Zhang, Guangxuan Xiao, Chuang Gan, and Song Han.
\newblock Qserve: W4a8kv4 quantization and system co-design for efficient llm serving, 2024{\natexlab{b}}.
\newblock URL \url{https://arxiv.org/abs/2405.04532}.

\bibitem[Shao et~al.(2024)Shao, Chen, Zhang, Xu, Zhao, Li, Zhang, Gao, Qiao, and Luo]{shao2024omniquantomnidirectionallycalibratedquantization}
Wenqi Shao, Mengzhao Chen, Zhaoyang Zhang, Peng Xu, Lirui Zhao, Zhiqian Li, Kaipeng Zhang, Peng Gao, Yu~Qiao, and Ping Luo.
\newblock Omniquant: Omnidirectionally calibrated quantization for large language models, 2024.
\newblock URL \url{https://arxiv.org/abs/2308.13137}.

\bibitem[Zhao et~al.(2024)Zhao, Lin, Zhu, Ye, Chen, Zheng, Ceze, Krishnamurthy, Chen, and Kasikci]{zhao2024atomlowbitquantizationefficient}
Yilong Zhao, Chien-Yu Lin, Kan Zhu, Zihao Ye, Lequn Chen, Size Zheng, Luis Ceze, Arvind Krishnamurthy, Tianqi Chen, and Baris Kasikci.
\newblock Atom: Low-bit quantization for efficient and accurate llm serving, 2024.
\newblock URL \url{https://arxiv.org/abs/2310.19102}.

\bibitem[Ashkboos et~al.(2024)Ashkboos, Mohtashami, Croci, Li, Jaggi, Alistarh, Hoefler, and Hensman]{ashkboos2024quarotoutlierfree4bitinference}
Saleh Ashkboos, Amirkeivan Mohtashami, Maximilian~L. Croci, Bo~Li, Martin Jaggi, Dan Alistarh, Torsten Hoefler, and James Hensman.
\newblock Quarot: Outlier-free 4-bit inference in rotated llms, 2024.
\newblock URL \url{https://arxiv.org/abs/2404.00456}.

\bibitem[Taori et~al.(2023)Taori, Gulrajani, Zhang, Dubois, Li, Guestrin, Liang, and Hashimoto]{alpaca}
Rohan Taori, Ishaan Gulrajani, Tianyi Zhang, Yann Dubois, Xuechen Li, Carlos Guestrin, Percy Liang, and Tatsunori~B. Hashimoto.
\newblock Stanford alpaca: An instruction-following llama model.
\newblock \url{https://github.com/tatsu-lab/stanford_alpaca}, 2023.

\bibitem[Dettmers et~al.(2023)Dettmers, Pagnoni, Holtzman, and Zettlemoyer]{dettmers2023qloraefficientfinetuningquantized}
Tim Dettmers, Artidoro Pagnoni, Ari Holtzman, and Luke Zettlemoyer.
\newblock Qlora: Efficient finetuning of quantized llms, 2023.
\newblock URL \url{https://arxiv.org/abs/2305.14314}.

\end{thebibliography}


==> sections/bi_smoothing.tex <==

\newtheorem{theorem}{Theorem}[section]


\section{A Bi-smoothing Strategy}

In~\cite{xiao2024smoothquantaccurateefficientposttraining}, it was proposed to mitigate activation outliers by reducing the maximum absolute values of activations while amplifying the maximum absolute values of weights. This approach assumes that activation outliers are concentrated in certain channels and are significantly more severe than weight outliers. However, as demonstrated in previous sections, this assumption no longer holds for the LLaMA3-70B and LLaMA3.1-70B model series, including their instruction-tuned versions. In this section, we introduce bi-directional smoothing algorithms that balance the magnitudes of both weights and activations.

\subsection{Equivalence in bi-directional smoothing}
Let $W\in \mathbb{R}^{M\times N}$ be the weights and $A \in \mathbb{R}^{B\times L\times N}$ be the input activation. In the representation of a Transformer linear layer, $M$ is output dimension, $N$ is the hidden dimension, $B$ is the batch size and $L$ is the sequence length. The output of the linear layer $Y \in \mathbb{R}^{B\times L\times M}$ is calculated by
\[
Y[i,:,:] = A[i,:,:] W^T, \forall 0\leq i \leq B-1,
\]
where we use Python tensor representation for the 3D tensor $A$, $Y$ and 2D tensor $W$.

There is an equivalence when multiplying $A[i,:,:]$ and $W$. 
\begin{theorem}
Let $S\in \mathbb{R}^{N}$ be a non-zero vector. We denote $W_s$ and $A_s$ the column-wise (last dimension) smoothed tensors, respectively, such that
$$
W_s[j,k] = W[j,k] S[k],  \forall 0\leq j \leq M, 0 \leq k \leq N-1,
$$
and
$$
A_s[i,j,k] = A[i,j,k] / S[k], \forall 0\leq i\leq B-1, 0\leq j\leq L-1,  0 \leq k \leq N-1,
$$
Then the following equation holds,
\[
A[i,:,:] W^T = A_s[i,:,:] W_s^T , \forall 0\leq i \leq B-1.
\]
\end{theorem}
\begin{proof}
Let $Y[i,:,:]=A[i,:,:] W^T$ and $Y_s[i,:,:]=A_s[i,:,:] W_s^T$, then $ \forall 0\leq i\leq B-1, 0\leq j\leq L-1,  0 \leq k \leq M-1$,
\begin{align*}
    Y_s[i,j,k] &= \sum_z A_s[i,j,z] W_s[z,j] \\
               &= \sum_z  A[i,j,z] / S[z] * W[z,j] S[z] \\
               &= \sum_z A[i,j,z] W[z,j] \\
               & = Y[i,j,k].
\end{align*}
\end{proof}
We call the vector $S\in \mathbb{R}^{N}$ the \textbf{smooth-factor} for $A$ and $W$.

\subsection{How to select the smooth-factor?}
For per-channel quantization, a quantization group consists of $N$ numbers and the max\_abs in the quantization group determines the scale-factor and quantization interval. First, assume the batch size is 1, and then $A\in \mathbb{R}^{1\times L \times N}$. Since it is desirable to minimize the max\_abs of both weight  and input activation, but the multiplication of these two values, i.e., $\max \left( \lvert W[:,i] \rvert \right)$ and $\max \left( \lvert A[0,:,i]\rvert \right)$, remains constant to guarantee the output of $A W^T$ is unchanged. Therefore, we choose the smooth-factor as
\begin{align*}
    S[k] = \sqrt{\frac{\max_j \left( \lvert A[0,j,k]\rvert \right)}{\max_j \left( \lvert W[j,k] \rvert \right)}}, \forall 0 \leq k \leq N-1.
\end{align*} 
Then we have
\begin{align*}
     \max_j \left( \lvert W_s[j,k] \rvert \right)&=  \max_j \left( \lvert W[j,k] S[i] \rvert \right) \\
     &=\sqrt{\max_j \left( \lvert A[0,j,k]\rvert \right) \max_j\left( \lvert W[j,k] \rvert \right)} \\
     &= \max_j \left( \lvert A[0,j,k] S[k]\rvert \right) \\
     & = \max_j \left( \lvert A_s[0,j,k] \rvert \right),
\end{align*}
i.e., the max\_abs after the bi-smoothing for weight and input activation is balanced. 
%This intuitively is optimal when the weight and input activation is quantized to the same number of bits.

In general when the batch size $B$ is greater than 1, then we can choose $S[k]$ as
  \begin{align}  \label{eq:smooth-factor}
    S[k] = \sqrt{\frac{\textrm{median}_i \max_j \left( \lvert A[i,j,k]\rvert \right)}{\max_j \left( \lvert W[j,k] \rvert \right)}}, \forall 0 \leq k \leq N-1.
\end{align}


\subsection{Main experiment results for bi-smoothing}

We show the accuracy comparison of all four LLaMA3-70B series of models (LLaMA3.1-70B-Instruct, LLaMA3.1-70B, LLaMA3-70B-Instruct, and LLaMA3-70B) in the section.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{LaTeX/figures/llama3-70b-w8a8-bi-smooth-is-good.png}
    \caption{Accuracy comparison of LLaMA3-70B model series with bi-smoothing}
    \label{fig:llama3.1-70b-bismooth}
\end{figure}

Figure~\ref{fig:llama3.1-70b-bismooth} demonstrates the effectiveness of the proposed bi-smoothing method for the entire LLaMA3-70B model series. It is observed that the  accuracy  of  models with per-channel W8A8  quantization are as good as their FP16 counterparts, which shows significant improvement over W8A16 models in Figure~\ref{fig:llama3-70b-w8a8}.  Note that to calculate the smooth-factor in Equation~(\ref{eq:smooth-factor}), we need some calibration data to estimate $\textrm{median}_i \max_j \left( \lvert A[i,j,k]\rvert \right)$. To prevent data contamination, we use only eight questions from the GPQA reasoning task for estimation. The calibration process takes only a few seconds, requiring a single inference pass over these samples. As demonstrated in the later ablation studies, the accuracy of the bi-smoothing method remains stable across varying amounts and sources of calibration data.


\subsubsection{Why bi-smoothing works well? }
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/bi-smooth-w_a_before-after.pdf}
    \caption{The plot illustrates the absolute values of weights and input activations in the LLaMA3.1-70B-Instruct model, specifically focusing on the first Q matrix in the initial Transformer block. The input activations are multiplied by the Q matrix. \textbf{Top-left}: Before bi-smoothing, large weight values (ranging from 60 to 80) form distinct "walls" parallel to the output axis. \textbf{Top-right}: After bi-smoothing, these weight "walls" remain but with significantly reduced magnitudes (below 2.0). \textbf{Bottom-left}: Input activations before bi-smoothing. \textbf{Bottom-right}: After bi-smoothing, the input activations are also suppressed, exhibiting smaller magnitudes.
}
    \label{fig:before-and-after-bi-smooth}
\end{figure}

Figure~\ref{fig:before-and-after-bi-smooth} compares the weights and input activations of the first Q matrix in the LLaMA3.1-70B-Instruct model. The input activations are drawn from a sequence of length 243 in the PIQA dataset. Notably, problematic weight outliers, with magnitudes exceeding 60, are suppressed to below 2.0, alongside activation outliers. This smoothing process makes both weights and activations far more resilient to quantization, achieving W8A8 accuracy nearly identical to that of the W16A16 configuration (as detailed in the next section).

In general, Figure~\ref{fig:qe_max_llama3-1-70b-inst-bi-smoothed} illustrates the quantization error and max\_abs across all layers of the LLaMA3.1-70B-Instruct model after bi-smoothing. Compared to Figure~\ref{fig:qe_max_llama3-70b}, depicting the unsmoothed model, there is a substantial reduction in max\_abs, yielding an order-of-magnitude decrease in quantization error.



\begin{figure} [h]
    \centering
    \includegraphics[width=0.8\linewidth]{LaTeX/figures/llama3.1-70b-inst-scaledW-w8-maxabs-qe.png}
    \caption{Quantization error and max\_abs of weights after bi-smoothing of each layer in the LLaMA3.1-70B-Instruct model.}
    \label{fig:qe_max_llama3-1-70b-inst-bi-smoothed}
\end{figure}

\subsection{Ablation study on bi-smoothing}

From Figure~\ref{fig:llama3.1-70b-bismooth}, we can see the best performing model is LLaMA3.1-70B-Instruct. So, we use this model for ablation study of bi-smoothing algorithms. We will show the bi-smoothing method is stable in calibration data and the choice of computing the smooth-factor.

\subsubsection{Calibration data source}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/llama3.1-70b-inst-w8a8-bi-smooth-gpqa-wg-pq.png}
    \caption{Different calibration data for bi-smoothing}
    \label{fig:calib-data-gpqa-wg-pq}
\end{figure}

Figure~\ref{fig:calib-data-gpqa-wg-pq} presents an accuracy comparison across different calibration data sources. We tested 8 samples from the GPQA dataset, 32 samples from the WG dataset, and 32 samples from the PQ dataset. The results indicate that the choice of calibration data has minimal impact on accuracy; all three datasets enable the W8A8 per-channel quantized model to achieve accuracy comparable to that of the FP16 counterpart.

\subsubsection{Calibration data size}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/llama3.1-70b-inst-w8a8-bi-smooth-gpqa-8sample-1sample.png}
    \caption{Comparison of calibration data using 8 samples and 1 sample from GPQA.}
    \label{fig:ablation_num_samples}
\end{figure}

We evaluated the impact of calibration data volume on smooth-factor computation, comparing results from 8 samples versus a single sample from the GPQA dataset. Figure~\ref{fig:ablation_num_samples} demonstrates that the difference in performance is negligible; both resulting W8A8 models achieve accuracy comparable to their FP16 counterpart.

\subsubsection{Smooth-factor calculation}

Note that in Equation (\ref{eq:smooth-factor}), we use ``median'' to calculate the smooth-factor. A natural alternative is to replace ``median'' by ``maximum''  in the following equation.
  \begin{align}  \label{eq:smooth-factor-alternative}
    S[k] = \sqrt{\frac{\max_i \max_j \left( \lvert A[i,j,k]\rvert \right)}{\max_j \left( \lvert W[j,k] \rvert \right)}}, \forall 0 \leq k \leq N-1.
\end{align}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/llama3.1-70b-inst-w8a8-bi-smooth-equations.png}
    \caption{Comparison of using Eq.~\ref{eq:smooth-factor} and Eq.~\ref{eq:smooth-factor-alternative} to calculate the smooth-factor}
    \label{fig:ablation-smooth-factor-calculation}
\end{figure}

Figure~\ref{fig:ablation-smooth-factor-calculation}  illustrates the comparison, revealing that there is negligible difference between using the ``median'' or ``max'' to calculate the smooth factor. This finding underscores the robustness of the bi-smoothing method in recovering the accuracy of W8A8 models.

\subsubsection{Applying bi-smoothing to a subset of Transformer layers}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/llama3.1-70b-inst-w8a8-bi-smooth-sub-block.png}
    \caption{ Applying bi-smoothing methods to a subset of Transformer blocks}
    \label{fig:ablation_subblock}
\end{figure}
%We have observed in previous section that only the first few Transformer blocks exhibit large weight outliers. We did ablation study on the number of blocks with bi-smoothing. Figure~\ref{fig:ablation_subblock} shows this comparison. When applying the bi-smoothing to only the first four Transformer blocks, it is observed that the accuracy of W8A8 can almost match the all-FP16 counterparts. This again verifies that the first few blocks are the root cause of the vulnerability of LLaMA3-70B model series against W8A8 quantization.

Our previous analysis revealed that significant weight outliers are predominantly confined to the initial Transformer blocks. An ablation study on the number of blocks with bi-smoothing method was conducted, with results illustrated in Figure~\ref{fig:ablation_subblock}. Notably, applying bi-smoothing to only the 0th, 1st, and 3rd Transformer blocks yields W8A8 accuracy nearly equivalent to that of the full-precision (FP16) model. This finding corroborates our hypothesis that the initial blocks are the primary source of the LLaMA3-70B model series' susceptibility to W8A8 quantization.



==> sections/main_file.tex <==
\section{Introduction}

The rising popularity of large language models (LLMs)~\cite{vaswani2023attentionneed,brown2020languagemodelsfewshotlearners,devlin2019bertpretrainingdeepbidirectional,liu2019robertarobustlyoptimizedbert,touvron2023llamaopenefficientfoundation} in diverse practical applications underscores their revolutionary impact on natural language processing, data analysis, and artificial intelligence. However, their immense size imposes a substantial burden on GPU memory~\cite{kaplan2020scalinglawsneurallanguage}, complicating deployment in resource-constrained environments. Quantization is a pivotal technique to mitigate this issue, reducing the memory footprint of LLMs while maintaining accuracy~\cite{gholami2021surveyquantizationmethodsefficient,Zafrir_2019,wang2023bitnetscaling1bittransformers}. By converting high-precision weights and activations to lower-precision formats, quantization facilitates more efficient model storage and accelerates inference. As the demand for LLMs grows, the advancement of quantization methods will be crucial for their scalable and cost-effective deployment in real-world applications.


Quantization uses lower precision to represent weights and activations. In this study, we focus on post-training integer-bit quantization (PTQ). The 8-bit weights and 8-bit activations (W8A8) configuration is often regarded as a good balance between efficiency and accuracy. Compared to the FP16 counterpart, W8 can save reduce the memory consumption and transaction by 50\%. Although 4-bit weights and 16-bit activations (W4A16) require even less memory, they often lack broad hardware support for the INT4-FP16 matrix-multiplication compute cores. In contrast, existing INT8-INT8 compute cores offer superior acceleration for the inference of W8A8 models. On the other hand, while the W4A4 configuration may reduce memory usage and latency through INT4-INT4 compute cores, it typically suffers from significant accuracy degradation due to the aggressive quantization. 

The granularity of a quantization group in large language models (LLMs) is another critical factor influencing the accuracy-acceleration trade-off. Within a quantization group, all values share the same scaling factor and zero point. When the group size matches the input dimension of a layer, this is termed ``per-channel'' quantization, which maximizes potential speedup. Conversely, ``per-group'' quantization occurs when an input channel is divided into multiple groups. This requires the intermediate partial sums of matrix-matrix multiplication to be transferred out of the compute cores, significantly reducing system throughput. Therefore, maintaining accuracy with per-channel quantization is essential for practical applications. 


In this paper, we investigate the W8A8 quantization for the most popular architectures and models featured on the LLM open leaderboard~\cite{open-llm-leaderboard}. Our study reveals a noteworthy phenomenon: the LLaMA3-70B model series~\cite{dubey2024llama3herdmodels} exhibits a pronounced vulnerability to W8A8 per-channel quantization, in stark contrast to other models, which demonstrate significantly greater robustness, typically experiencing less than 1\% accuracy degradation compared to their FP16 counterparts under the same quantization scheme. 
Our observation on the ``LLaMA3-70B series'' also include the LLaMA3.1-70B and various fine-tuned versions, and other robust models include LLaMA2 series, LLaMA3-8B, Mistral-123B, Mixtral-8x7B, Qwen2-72B, Phi3-13B, and Falcon-40B~\cite{jiang2023mistral7b,jiang2024mixtralexperts,yang2024qwen2technicalreport,abdin2024phi3technicalreporthighly,almazrouei2023falconseriesopenlanguage}.  Figure~\ref{fig:llama3-70b-w8a8} provides a comparative analysis of FP16 (labeled as W16A16) and W8A16 quantization for the officially released LLaMA3/3.1-70B and LLaMA3/3.1-70B-Instruct by Meta. This comparison reveals that significant accuracy degradation already occurs with W8A16, indicating that the issue primarily stems from weight quantization rather than activation quantization. Details will be presented in the experiment section. Released in April 2024, the LLaMA3-70B has not been extensively examined in recent research on W8A8 per-channel quantization. Given that this series is currently the most widely used base model on the open leaderboard, further exploration and understanding of its unique characteristics are imperative.


\begin{figure}[tbp]
    \centering

    \includegraphics[width=1\linewidth]{LaTeX/figures/llama3-70b-series-w8a16-is-bad.png}
    %{LaTeX/figures/llama3-70b-series-accuracy.png}
    \caption{Accuracy  of LLaMA3-70B model series with W16A16, and W8A16 per-channel quantization}
    
    \label{fig:llama3-70b-w8a8}
\end{figure}


To elucidate the unique vulnerability of the LLaMA3-70B series to W8A8 per-channel quantization, we conducted a comparative analysis of its weight distributions against those of other robust models. Our investigation revealed a significant discrepancy, particularly pronounced in the initial layers. These layers exhibit a distinctive characteristic wherein magnitudes of certain weights exceed others by several orders of magnitude. Figure~\ref{fig:wd_llama3-70b} shows an example of the ``V'' matrix in the first Transformer block of the LLaMA3-70B model. Weights with large magnitudes are concentrated on specific input dimensions, with the largest values exceeding 90.
These outlier weights substantially expand the quantization range, resulting in larger quantization intervals and consequently diminished precision for smaller weight values. Notably, these weight outliers are only prominent in the ``Q'', ``K'', ``V'', ``Up'', and ``Gate'' weight matrices of the initial transformer blocks, while the "O" and "Down" weight matrices do not exhibit this behavior. 
We propose two methods to address this issue. First, to mitigate these quantization errors, we propose implementing per-group quantization specifically for these affected layers. Although these layers constitute merely 2-3\% of the total layers in LLaMA3-70B, this targeted approach yields a dramatic enhancement in accuracy, elevating model performance to a level approaching that of FP16 models. Second, we demonstrate a bi-directional smoothing method of the weight and activation matrices that effectively reduces the dynamic range of both, significantly minimizing quantization errors. This technique preserves per-channel quantization while enhancing the model's resilience to W8A8 quantization.

\begin{figure}[tbp]
    \centering
    %\hspace{-2em}
    \includegraphics[width=0.7\linewidth]{LaTeX/figures/llama3-70b-v0-matrix.png}
    \caption{abs\_weights of the ``V'' matrix in the first Transformer block of LLaMA3-70B}
    \label{fig:wd_llama3-70b}
\end{figure}

The contribution of this paper is as follows.

\begin{itemize}
\item We show that the LLaMA3-70B model series has a unique characteristic that makes it the only model series on the open LLM leaderboard vulnerable to W8A8 per-channel post-training quantization (PTQ). In contrast, all other models can be safely quantized to per-channel-W8A8 with negligible accuracy loss. We believe this observation holds significant implications since LLaMA3-70B serves as one of the most popular base models for numerous models fine-tuned for domain-specific tasks.
\item We identify that LLaMA3-70B's sensitivity to per-channel PTQ stems from its significantly different weight distribution, particularly the presence of substantial weight outliers.
\item To address this, we first propose a mixed per-channel/per-group quantization strategy. This approach applies per-group quantization to less than 3\% of the layers, specifically those with significant weight outliers, while maintaining per-channel quantization for the remaining 97\% layers. This mixed strategy effectively restores the accuracy of the LLaMA3-70B model series to levels comparable to its FP16 counterparts.
\item The second method introduces bi-directional smoothing to mitigate outliers in both weights and input activations. This approach significantly reduces the dynamic range required for quantization, enabling the LLaMA3-70B model series to retain accuracy comparable to their FP16 counterparts.
\end{itemize}


\section{Quantization Basics}
In this paper, we use symmetric integer-bit quantization due to its high efficiency and simpler hardware support. In symmetric $n$-bit integer quantization, we map floating-point (FP) values to integers in $[-2^{n-1}, 2^{n-1}-1]$. This process involves scaling the FP values based on a scale-factor and an offset. This offset is sometimes called ``zero-point'' and is set to $0$ for symmetric quantization. 

Let \( x \) be a FP value, and \( x_q \) its quantized integer representation. The scale-factor \( s \) is determined by the range of the FP values and the desired range of the integers. The symmetric quantization formula is given by:

\[
x_q = \text{round}\left(\frac{x}{s}\right)
\]
where \( \text{round}(\cdot) \) rounds the result to the nearest integer.

The scale-factor \( s \) is typically calculated based on the maximum absolute value of the FP values, \( \text{max\_abs} \), and the maximum representable integer value, \( 2^{n-1}-1 \). For symmetric quantization, the scale-factor is defined as:

\[
s = \frac{\text{max\_abs}}{2^{n-1}-1 }
\]

Thus, the quantization and dequantization processes can be expressed as:

\[
x_q = \text{round}\left(\frac{x}{s}\right)
\quad \text{and} \quad
x \approx x_q \cdot s
\]

The scale-factor $s$ plays a crucial role in the quantization process. The number of floating-point values used to determine \text{max\_abs} is typically referred to as the group size. In LLMs, consider a weight matrix $W$ of dimension $M\times N$  and an input activation matrix $A$ of dimension $L\times N$. The resultant output of $A\cdot W^T$  has dimension $L\times M$. Here $L$, $N$, and $M$ represent the sequence length, hidden dimension, and output dimension in a Transformer layer, respectively.
For per-channel quantization of $W$, the group size is $N$, implying that each row of $N$ values in $W$ shares a common scale-factor. Consequently, all scale-factors form a vector of length $M$. Similarly, per-channel quantization of $A$ also has a group size of $N$, with each row of $N$ values in $A$ sharing a scale-factor, resulting in a scale-factor vector of length $L$.
This configuration enables the computation of floating-point matrix multiplication using integer-bit compute cores (e.g., INT8 tensor cores), followed by dequantization. The dequantization process involves an element-wise multiplication with the scale-factor matrix of dimension $L\times M$, derived as the outer product of the scale-factor vectors of $W$ and $A$. Notably, this dequantization can often be efficiently fused into the subsequent operation after $A\cdot W^T$ in LLMs, which is typically an element-wise operation such as rotary embedding, SiLU activation application, or normalization.
In contrast, per-group quantization of $W$ and $A$ employs a finer granularity, where each row of $W$ (and of $A$) is partitioned into groups, each with its own scale-factor. Consequently, the output $A\cdot W^T$ cannot be computed in a single cycle within the INT tensor core, as the scale-factors differ during accumulation in the multiply-accumulation (MAC) unit. This leads to a degradation in the compute efficiency of the quantized model.
Given these considerations, per-channel quantization is generally preferred unless the quantization-induced error degrades the model's accuracy to an unacceptable level.

\section{The Uniqueness of LLaMA3-70B with per-channel W8A8}
\label{sec:experiment-llama3-70b}

\subsection{Test Dataset}
\del{We tested LLM models on 8 reasoning tasks, namely, Hellaswag (HS), PIQA (PQ), OpenbookQA (OQ), ARC-easy (AE), Winogrande (WG), ARC-Challenge (AE), BoolQ (BQ), and MMLU~. We observe that many studies report the average accuracy over reasoning task by simply averaging the accuracy of each task, which might not be rigorous since the number of questions in each task has large variance. For example, HS and MMLU both have over 10K questions while OQ has only 500 questions. In order to take this into account, we also report the ``weighted average accuracy'' (denoted by WT-AVG in figures), which is the total number of correct answers divided by the total number of questions. In this way, the accuracy of dataset with a large number of questions is weighted more than smaller dataset.}

\claude{We evaluated LLMs across eight reasoning tasks: Hellaswag (HS), PIQA (PQ), OpenbookQA (OQ), ARC-Easy (AE), Winogrande (WG), ARC-Challenge (AC), BoolQ (BQ), and MMLU\cite{zellers2019hellaswagmachinereallyfinish,bisk2019piqareasoningphysicalcommonsense,OpenBookQA2018,allenai:arc,sakaguchi2019winograndeadversarialwinogradschema,clark2019boolqexploringsurprisingdifficulty,hendryckstest2021,hendrycks2021ethics}. We report the ``accuracy'' for all tasks. Some tasks have ``normalized accuracy'' and the conclusions derived from ``accuracy''  remain consistent when applied to ``normalized accuracy''. We realize that many studies report the average accuracy over these reasoning tasks by simply computing the arithmetic mean of individual task accuracies (denoted by ``AVG'' in our figures). However, this approach may lack rigor due to the significant variance in the number of questions across tasks. For instance, HS and MMLU each contain over 10,000 questions, while OQ comprises only 500.}

\claude{To address this disparity, we use an additional metric: the ``weighted average accuracy.'' This metric is calculated by dividing the total number of correct answers across all tasks by the total number of questions. Consequently, this method assigns greater weight to datasets with a larger number of questions, providing a more balanced representation of model performance across tasks of varying sizes. It is denoted by ``WT-AVG'' in our figures.}

\subsection{Tested Models}
We  test the  accuracy of the following models: LLaMA3-70B, LLaMA3-70B-Instruct, LLaMA3.1-70B, Llama3-70B-Synthia, calme-2.2-llama3-70b, LLaMA3-8B, LLaMA2-70B, LLaMA2-70B-chat, Qwen2-72B, Mixtral-8x7B, Phi3-14B-Instruct, Mistral-L-Instruct-123B, Falcon-40B.  HuggingFace links to them will be provided in the appendix. We also analyze the weight distribution of LLaMA3.1-405B without evaluating its accuracy with FP16 due to GPU memory limitations.

\subsection{Test Environments}
All tests are done within 8xA100 (80GB) GPUs with PyTorch framework using lm-evaluation-harness~\cite{eval-harness}. 

\subsection{LLaMA3-70B's sensitivity to W8A8 }


\begin{figure}[tbp]
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/llama3-70b-finetuned-w8a16-is-bad.png}
    %{LaTeX/figures/llama3_70b_finetuned_accu.png}
    \caption{W8A8 per-channel quantization accuracy of models using  LLaMA3-70B as the base model }
    \label{fig:llama3-70b-finetuned-w8a16}
\end{figure}


\claude{Figure~\ref{fig:llama3-70b-w8a8} and Figure~\ref{fig:llama3-70b-finetuned-w8a16} present a comparative analysis of accuracy for several models in the LLaMA3-70B series subjected to 8-bit per-channel post-training quantization. This analysis encompasses the recently released LLaMA3.1-70B and two additional models fine-tuned from LLaMA3-70B. }
\claude{
These figures yield several notable observations:
\begin{itemize}
    \item The accuracy of models undergoes significant degradation with W8 quantization, even when activations are maintained at FP16 precision. This indicates that the observed accuracy deterioration is not attributable to quantization errors in activations, but rather originates from the 8-bit weight quantization process.
    \item Models fine-tuned from LLaMA3-70B exhibit the same vulnerability to W8 quantization as their base model. This persistence of vulnerability can be attributed to the fact that fine-tuning typically induces only minor alterations to weight values. In the subsequent section, we will demonstrate that this vulnerability is intrinsically linked to the underlying weight distributions of the model.
\end{itemize}
}


\begin{figure}[hthp]
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/Other-Llama-w8a8-is-good.png}
    %{LaTeX/figures/llama-other-acc-mycmap.png}
    \caption{Accuracy of other LLaMA models  with W8A8 per-channel quantization}
    \label{fig:llama_else}
\end{figure}
  \begin{figure}[hthp]
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/Llama3.2-1b-3b-w8a8-is-good.png}
    %{LaTeX/figures/llama-other-acc-mycmap.png}
    \caption{LLaMA3.2 models with W8A8 per-channel quantization}
    \label{fig:llama_3.2}
\end{figure}
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/Qwen-and-Mistral-w8a8-is-good.png}
    %{LaTeX/figures/llm-other-acc-mycmap.png}
    \caption{Accuracy of other Transformer-based models with W8A8 per-channel quantization}
    \label{fig:qwen_mistral_model_acc}
\end{figure*}
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/Mixtral-Phi-Falcon-w8a8-is-good.png}
    %{LaTeX/figures/llm-other-acc-mycmap.png}
    \caption{Accuracy of other Transformer-based models with W8A8 per-channel quantization}
    \label{fig:mixtral_phi_falcon_model_acc}
\end{figure*}

\subsection{LLaMA3-70B  is the ONLY ONE sensitive to W8A8 }
Figure~\ref{fig:llama_else} , Figure~\ref{fig:qwen_mistral_model_acc} and Figure~\ref{fig:mixtral_phi_falcon_model_acc} compare the accuracy of other models with different architectures with W8A8  quantization. 
\claude{The analysis spans the LLaMA family, including LLaMA3-8B, LLaMA2-70B, and LLaMA2-70B-chat, as well as other prominent Transformer-based designs such as Qwen2-72B, Mixtral-8x7B, Mistral-123B, Phi3-13B, and Falcon-40B. These architectures represent the top-performing architectures in the LLM Open Leaderboard.}

The data presented in these figures illustrates a  contrast to the behavior observed in the LLaMA3-70B series. Specifically, the models examined here exhibit remarkable resilience to W8A8 per-channel quantization. In the majority of instances, the performance of W8A8 quantized versions closely approximates that of their FP16 counterparts. 
%While minor variations exist, the performance decline rarely exceeds 1.5\% (Mistral-123B).




\subsection{Why LLaMA3-70B is the only one?}

In order to understand the uniqueness of LLaMA3-70B models, we explore the weight distributions. 





  \begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{LaTeX/figures/llama3.1-70b-v0-matrix.png}
    \caption{abs\_weights of the V matrix in the first Transformer block of LLaMA3.1-70B}
    \label{fig:wd-llama3.1-70b}
\end{figure}


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{LaTeX/figures/llama2-70b-v0-matrix.png}
    \caption{abs\_weights of the V matrix in the first Transformer block of LLaMA2-70B}
    \label{fig:wd-llama2-70b}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\linewidth]{LaTeX/figures/llama3-8b-v0-matrix.png}
    \caption{abs\_weights of the V matrix in the first Transformer block of LLaMA3-8B}
    \label{fig:wd-llama3-8b}
\end{figure}


\subsubsection{A qualitative exploration}

Figures~\ref{fig:wd_llama3-70b},~\ref{fig:wd-llama3.1-70b},~\ref{fig:wd-llama2-70b}, and~\ref{fig:wd-llama3-8b}, illustrate the absolute values of the V matrix weights in the first Transformer block for LLaMA3-70B, LLaMA3.1-70B, LLaMA3-8B, and LLaMA2-70B models, respectively. Other weight matrices for other models show similar trend and are shown in the Appendix. It is important to note that in per-channel quantization, each group comprises a length-$N$ vector along the input dimension. Our analysis reveals several key observations:

\begin{itemize} 
\item The maximum absolute weight values (max\_abs) in LLaMA3-70B ($93$) and LLaMA3.1-70B ($92.5$) surpass those in LLaMA3-8B ($0.05$) and LLaMA2-70B ($0.07$) by approximately three orders of magnitude. Furthermore, LLaMA3/3.1-70B exhibits a non-trivial number of weights with large magnitudes along the output dimension, which we term ``weight outliers''. This extensive range of weight values results in large quantization intervals for LLaMA3/3.1-70B, leading to substantial quantization errors in groups containing any weight outliers.
\item LLaMA3-70B displays a distinct pattern where weights with large max\_abs values cluster at specific input indices, forming visible "walls" in Figure~\ref{fig:wd_llama3-70b} and~\ref{fig:wd-llama3.1-70b}. In contrast, LLaMA2-70B and LLaMA3-8B lacks such obvious patterning.
\end{itemize}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{LaTeX/figures/qerror_abs_max_llama3_70b_w_zoomin.png}
    \caption{Quantization error and max\_abs of weights in each layer in LLaMA3-70B. LLaMA3-70B-Instruct, LLaMA3.1-70B, and LLaMA3.1-70B-Instruct have similar patterns.}
    \label{fig:qe_max_llama3-70b}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{LaTeX/figures/qerror_abs_max_llama2_70b.png}
    \caption{Quantization error and max\_abs of weights in each layer in LLaMA2-70B}
    \label{fig:qe_max_llama2-70b}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{LaTeX/figures/qerror_abs_max_llama3_8b.png}
    \caption{Quantization error and max\_abs of weights in each layer in LLaMA3-8B}
    \label{fig:qe_max_llama3-8b}

\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{LaTeX/figures/qerror_abs_max_llama3_1_405b.png}
    \caption{Quantization error and max\_abs of weights in each layer in LLaMA3.1-405B}
    \label{fig:qe_max_llama3-1-405b}
\end{figure}


\subsubsection{A quantitative exploration}

\claude{To quantitatively assess the robustness of weights under W8 quantization, we employ two key metrics. The first is the maximum absolute value (max\_abs) of weights for each layer in the model, which determines the scale factor and, consequently, the quantization interval. The second metric is the quantization error, measured by the root-mean-square error (RMSE) between the FP16 and 8-bit weights. These metrics are positively correlated, as larger quantization intervals typically result in greater errors.}

\claude{Figure~\ref{fig:qe_max_llama3-70b}, ~\ref{fig:qe_max_llama2-70b},~\ref{fig:qe_max_llama3-8b},~\ref{fig:qe_max_llama3-1-405b}  illustrate the max\_abs and quantization error for four LLaMA models: LLaMA3-70B, LLaMA2-70B, LLaMA3-8B, and the recently released LLaMA3.1-405B. The x-axis represents the total number of layers, excluding the initial embedding layer and the final output head. Each Transformer block in a LLaMA model comprises seven matrices (Q, K, V, O, up, gate, down), with 80, 80, 32, and 126 blocks in the four models, respectively. The left y-axis denotes the quantization error, while the right y-axis indicates the max\_abs weight of each layer.

}

Our comprehensive analysis of weight distributions across various layers and different LLM models yields the following conclusions:
\begin{itemize}
    \item In the initial layers, the LLaMA3-70B model exhibits weight outliers with max\_abs values that surpass those of its latter layers and all layers in other models by orders of magnitude. See the subfigure in Figure~\ref{fig:qe_max_llama3-70b} for a zoom-in view of the first 98 layers (14 blocks). This results in significantly larger quantization intervals, leading to quantization errors that are 1-2 orders of magnitude greater than in other models or layers.
    \item In the latter layers, the LLaMA3-70B model demonstrates behavior similar to other models in terms of quantization errors and max\_abs of weights. This observation suggests that the sensitivity of the LLaMA3-70B model series to W8 quantization may primarily stem from the initial layers. We will provide further confirmation of this hypothesis in the subsequent section.
\end{itemize}




\section{A Mixed Grouping Strategy}

\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/llama3-70b-series-w8a8-mix-grouping-is-good.png}
    %{LaTeX/figures/llama3-70b-mix-group-1024.png}
    \caption{Accuracy comparison of  LLaMA3-70 model series with mixed grouping}
    \label{fig:llama3_70b_mixed_grouping}
\end{figure*}
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{LaTeX/figures/llama3-70b-derivatives-w8a8-mix-grouping-is-good.png}
    %{LaTeX/figures/llama3-70b-mix-group-1024.png}
    \caption{Accuracy comparison of  LLaMA3-70 derivative models with mixed grouping}
    \label{fig:llama3_70b_derivative_mixed_grouping}
\end{figure*}


Based on our analysis of Figure~\ref{fig:qe_max_llama3-70b} , we have empirically identified that in the LLaMA3-70B model, the Q, K, V, Up, and Gate matrices of Block 0, 1, and 3 exhibit exceptionally high quantization errors and maximum absolute weight values. To mitigate these quantization errors, we propose implementing a finer grouping granularity specifically for these 15 layers.

It is noteworthy that the layers requiring per-group quantization, as opposed to per-channel quantization, constitute only 2.68\% (15/560) of the total layers in the model. While many quantization studies employ group sizes of 128 or smaller (e.g., GPTQ, AWQ), our investigation reveals that a group size of 1024 is sufficient to prevent accuracy degradation while maintaining a larger group size for improved hardware efficiency.

\subsection{Main experimental results on mixed grouping}
Figure~\ref{fig:llama3_70b_mixed_grouping}  and Figure~\ref{fig:llama3_70b_derivative_mixed_grouping} presents a comparative analysis of the accuracy achieved by our proposed method against that of FP16 models. The presented models includes several LLaMA3-70 and its variants and derivatives in the Open LLM Leaderboard. The results convincingly demonstrate that our mixed quantization approach—combining 2.68\% per-group and 97.32\% per-channel 8-bit quantization—can match the accuracy of the LLaMA3-70B model with FP16 precision.

%Figure~\ref{fig:qe_comparison_mix} illustrates the significant reduction in quantization errors achieved for the initially affected layers (specifically, the Q, K, V, Up, and Gate matrices of Blocks 0, 1, and 3) through the implementation of per-group quantization with a group size of 1024. While the maximum absolute value (max\_abs) for each layer remains unchanged, the reduction in the number of quantized values per group leads to a marked decrease in quantization error.

This improvement can be attributed to the finer granularity of the quantization process in these critical layers. By reducing the group size from the entire channel to 1024 elements, we effectively create multiple quantization groups within each channel. This approach allows for more precise representation of weight values, particularly in the presence of outliers that previously dominated the quantization scale factors.


In summary, this hybrid quantization strategy effectively addresses the unique challenges posed by the LLaMA3-70B model's weight distribution, particularly in its initial layers, while minimizing the hardware complexity overhead associated with per-group quantization across the entire model.


    \begin{comment}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.7\linewidth]{LaTeX/figures/qerror_comparison_with_mixed_group_1024vsnogrouping.png}
    \caption{Quantization error reduction by size-1024 grouping. Only layers in the first 4 Transformer blocks (28 layers) in LLaMA3-70B are displayed. }
    \label{fig:qe_comparison_mix}
\end{figure}

\end{comment}
%\section{Ablations}

\begin{comment}
    

\section{Other Tasks and Experiment}

Building upon our analysis of the LLaMA3-70B series' distinctive behavior across eight reasoning tasks and the efficacy of our mixed grouping strategy in restoring accuracy, we extend our investigation to the domain of mathematics. Specifically, we evaluate performance on the GSM8k task using 8-shot Chain-of-Thought (CoT) prompting.

Our experimental protocol encompasses four models previously identified as susceptible to W8 quantization, alongside two models demonstrating robustness to per-channel W8A8 quantization. The results, presented in Table~\ref{tab:gsm8k_acc}, reveal that the mathematical capabilities of the LLaMA3-70B series are similarly compromised by W8 quantization, mirroring the degradation observed in other cognitive tasks.

Crucially, our findings indicate that the proposed mixed grouping method—employing size-1024 per-group quantization for those 15 sensitive layers—proves equally effective in recovering accuracy on this mathematical task. This consistency across diverse cognitive domains underscores the generalizability of our quantization strategy and its potential to preserve model performance across a broad spectrum of language understanding and reasoning tasks.



\begin{table}[h!]
\centering
\begin{tabular}{l|c|c|c}
\toprule
Model & W16A16 & W8A8-m-g& W8A8\\ \hline 
LLama3-70B-Inst& 0.9037& 0.8961& xxxx\\ \hline 
LLama3.1-70B-Inst& 0.9174& 0.9181& xxxx\\
\end{tabular}
\caption{Accuracy of GSM8K under different quantization configurations.}
\label{tab:gsm8k_acc}
\end{table}

\end{comment}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{LaTeX/figures/mix_group_size_ablation.png}
    %{LaTeX/figures/llama3_MGsize_ablation.png}
    \caption{Ablation study on the mixed group size for Q, K, V, Up, and Gate of Block 0, 1, 3 in LLaMA3-70B}
    \label{fig:llama3_70b_MG_ablation}
\end{figure}

\subsection{Ablation on the group size}
We examine the influence of varying group sizes on the accuracy of W8A8 quantization for the LLaMA3-70B model. Figure~\ref{fig:llama3_70b_MG_ablation} illustrates this comparative analysis. Our results reveal that certain datasets, notably AE, AC, and OQ, exhibit particular sensitivity to increased group size applied exclusively to a total of 15 layers within Blocks 0, 1, and 3. From a holistic perspective, per-group quantization employing sizes of 512 or 1024 emerges as a good compromise between model accuracy and hardware efficiency. 


\input{LaTeX/sections/bi_smoothing}

\begin{comment}
    

\begin{table}[h!]
\centering
\begin{tabular}{l|c|c|c}
\toprule
Group size& 256& 512& 1024\\ \hline 
Weighted Average& 0.733& 0.732& 0.733\\ \hline 
Average& 0.713& 0.710& 0.708\\
\bottomrule
\end{tabular}
\caption{Ablation study on the mixed group size for Q, K, V, Up, and Gate of Block 0, 1, 3 in LLaMA3-70B}
\label{tab:gsm8k_acc}
\end{table}

\end{comment}

\section{Discussions}

According to Meta's technical report~\cite{dubey2024llama3herdmodels}, LLaMA2-70B and LLaMA3-70B share similar model architectures, while LLaMA3-8B/70B and LLaMA3.1-8B/70B/405B are reported to have similar training data and strategies. However, our analysis reveals significantly different weight distribution characteristics in LLaMA3/3.1-70B compared to other LLaMA models. This unexpected divergence in weight patterns, particularly the presence of numerous large outliers exclusively in LLaMA3/3.1-70B models, presents an intriguing peculiarity.

The origins of this phenomenon remain unclear, given that models sharing either architectural design or training methodologies do not exhibit similar characteristics. Unraveling the underlying mechanisms responsible for this unique weight distribution could potentially offer valuable insights into the learning processes of Large Language Models (LLMs), especially in the context of reasoning tasks.

\input{LaTeX/sections/related_work}



\section{Conclusions}
Our investigation reveals a distinctive vulnerability in the LLaMA3-70B model series, including LLaMA3.1-70B, to per-channel quantization. We attribute this susceptibility to significant weight outliers in the initial layers. The contrast in behavior between the LLaMA3-70B and other LLaMA models (LLaMA2, LLaMA3/3.1-8B, LLaMA3.1-405B), as well as other tested LLMs with different architectures, warrants further exploration of the underlying training strategies. To address this issue, we propose a mixed-grouping method that substantially enhances the accuracy of LLaMA3-70B from 45.4\% to 73.4\%, effectively matching the performance of its FP16 counterpart.

%We demonstrate a unique behavior of LLaMA3-70 model series (including LLaMA3.1-70B) that are susceptible to per-channel quantization, and we conclude that it is caused by significant weight outliers in the initial few layers. Considering that all other LLaMA series (all LLaMA2 models, LLaMA3/3.1-8B, and LLaMA3.1-405B) and all other LLM models tested behave quite different from LLaMA3-70B series, we believe it is worthwhile to explore the training strategies for a deep understanding. We also propose a mixed-grouping method to enhance the accuracy of the LLaMA3-70B from 45\% to 73\% and match the accuracy of the LLaMA3-70B FP models.


\clearpage



==> sections/related_work.tex <==
\section{Related Works}
Quantization is useful in reducing model size and potentially increases model inference speed~\cite{han2016deepcompressioncompressingdeep,jacob2017quantizationtrainingneuralnetworks,nagel2019datafreequantizationweightequalization,bondarenko2021understandingovercomingchallengesefficient,wang2019haqhardwareawareautomatedquantization,bengio2013estimatingpropagatinggradientsstochastic}. There two main categories of quantization, post-training quantization (PTQ) and quantization-aware training (QAT).
\subsection{Post-training quantization}
PTQ does not use any back-propagation to finetune weights. For \textbf{weight-only quantization}, LLM.int8()~\cite{dettmers2022llmint8} uses a mixed precision with 16-bit MAC for outliers. GPTQ~\cite{frantar2023gptq} and AWQ~\cite{lin2023awq} quantize the per-group weight-only tensor using as small as 3-4 bits. SqueezeLLM~\cite{kim2024squeezellmdenseandsparsequantization} uses non-uniform quantization and store outliers efficiently. For~\textbf{weight-activation quantization} that enables faster inference~\cite{dettmers2022gptint,wei2023outliersuppressionpushinglimit} 
SmoothQuant~\cite{xiao2024smoothquantaccurateefficientposttraining} transfers the outliers from activation to weights to enable per-tensor W8A8. 
QServe~\cite{lin2024qservew4a8kv4quantizationcodesign} proposes W4A8K4 to serve LLM models.
Some other studies enable even smaller number of bits~\cite{shao2024omniquantomnidirectionallycalibratedquantization, zhao2024atomlowbitquantizationefficient, ashkboos2024quarotoutlierfree4bitinference}. 
Notably, our observations on the weights and activations of the LLaMA3-70B model series contrast with those of SmoothQuant. The proposed bi-smoothing method extends this approach by addressing both weight and activation outliers. Compared to other PTQ methods, we aim to maintain per-channel  instead of per-group quantization for maximal hardware efficiency.

\subsection{Quantization aware training}
Quantization-aware training (QAT) requires both calibration data and  back-propagation to finetune the quantize weights~\cite{bengio2013estimatingpropagatinggradientsstochastic,gholami2021surveyquantizationmethodsefficient}. While full finetuning~\cite{alpaca} can recover the accuracy to the maximum extent, Q-LoRA~\cite{dettmers2023qloraefficientfinetuningquantized} reduces the memory requirement significantly.
